Learning to Take Directions One Step at a Time

We present a method to generate a video sequence given a single image. Because items in an image can be animated in arbitrarily many different ways, we introduce as control signal a sequence of motion strokes. Such control signal can be automatically transferred from other videos, e.g., via bounding box tracking. Each motion stroke provides the direction to the moving object in the input image and we aim to train a network to generate an animation following a sequence of such directions. To address this task we design a novel recurrent architecture, which can be trained easily and effectively thanks to an explicit separation of past, future and current states. As we demonstrate in the experiments, our proposed architecture is capable of generating an arbitrary number of frames from a single image and a sequence of motion strokes. Key components of our architecture are an autoencoding constraint to ensure consistency with the past and a generative adversarial scheme to ensure that images look realistic and are temporally smooth. We demonstrate the effectiveness of our approach on the MNIST, KTH, Human3.6M, Push and Weizmann datasets.

==> figures/fid.tex <==
\begin{table}
	\footnotesize 
	\caption{
		Comparison of LPIPS~\cite{zhang2018unreasonable} between generated and test set distribution of the last predicted (16-th) frame. Smaller values are better.
		%$^\ast$Li \etal have released their code, but not the model weights for KTH. 
		%We re-trained their model, but were not able to reproduce the quality they show in the paper.
		\label{tbl:quantitative-fid}
	}
	\centering
	\setlength{\tabcolsep}{8.5pt}
	\begin{tabular}{lrrr}
		\toprule
								& Li \etal~\cite{li2018flow}		& Denton \etal~\cite{denton2018stochastic}	& Ours	 \\
		\midrule
		%FID						& -									& 55.6										& \textbf{26.0} \\
		LPIPS					& 0.14								& 0.11										& \textbf{0.09} \\
		\bottomrule
	\end{tabular}
	%\vspace{-2mm}
\end{table}


==> figures/kth_1.tex <==
\begin{figure*}
	\centering
	\begin{subfigure}[b]{\textwidth}
		\setlength\tabcolsep{0.1pt}
		\begin{tabular}{p{0.065\textwidth}p{0.065\textwidth}p{0.92\textwidth}}
			{\small Stroke} & {\small Image} &   \\
			\includegraphics[width=0.0564\textwidth]{./images/kth/ex1/stroke.png}&
			\includegraphics[width=0.0566\textwidth]{./images/kth/ex1/input.png}&
			\includegraphics[width=0.85\textwidth]{./images/kth/ex1/frame.png}\\
		\end{tabular}
	\end{subfigure}\\
	\begin{subfigure}[b]{\textwidth}
		\setlength\tabcolsep{0.1pt}
		\begin{tabular}{p{0.065\textwidth}p{0.065\textwidth}p{0.92\textwidth}}
			{\small Stroke} & {\small Image} &   \\
			\includegraphics[width=0.0564\textwidth]{./images/kth/ex2/stroke.png}&
			\includegraphics[width=0.0566\textwidth]{./images/kth/ex2/input.png}&
			\includegraphics[width=0.85\textwidth]{./images/kth/ex2/frame.png}\\
		\end{tabular}
		\vspace{-1mm}
\end{subfigure}
%\setlength{\tabcolsep}{100cm}
    \caption{
    \label{fig:results-kth} 
    \textbf{Experiments on the KTH dataset.} 
    For each row, the first column is the input stroke where the intensity of the point goes from black to light grey over time. 
    The second column is the input image. 
    Starting from the third column to the end are the frames from the generated sequence.
    }
\end{figure*}

==> figures/mnist_1.tex <==
\begin{figure*}
	\centering
	\small
	\def\arraystretch{0.1}	
	\newcommand{\height}{4.00cm}
	\newcommand{\vheight}{0.251\height}
	\newcommand{\vsep}{0.05mm}
	% Figure (a)
   	\begin{subfigure}[b]{\textwidth}
		\setlength\tabcolsep{1pt}
		\begin{tabular}{lll}
			{\small Stroke} & {\small Image} & \\
			\includegraphics[height=\height]{./images/mnist/a-new/stroke-repeated.png} &
			\includegraphics[height=\height]{./images/mnist/a-new/input.png}&
			\includegraphics[height=\height]{./images/mnist/a-new/frame-without-input-last.png} 
		\end{tabular}%
		\setlength\tabcolsep{0.0pt}%
		\begin{tabular}{l}
			{\small Video }
			\vspace{0.5mm} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/a-new/1/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/a-new/2/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/a-new/3/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/a-new/4/frame}{001}{016} \\
		\end{tabular}
		\caption{}
	\end{subfigure}
	% Figure (b)
	\begin{subfigure}[b]{\textwidth}
		\setlength\tabcolsep{1pt}
		\begin{tabular}{lll}
			{\small Stroke} & {\small Image} & \\
			\includegraphics[height=\height]{./images/mnist/b-new/mnist-full-stroke.png} &
			\includegraphics[height=\height]{./images/mnist/b-new/mnist-full-input.png}&
			\includegraphics[height=\height]{./images/mnist/b-new/mnist-without-input-last.png} 
		\end{tabular}%
		\setlength\tabcolsep{0.0pt}%
		\begin{tabular}{l}
			{\small Video }
			\vspace{0.5mm} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/b-new/1/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/b-new/2/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/b-new/3/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/b-new/4/frame}{001}{016} \\
		\end{tabular}
		\caption{}
	\end{subfigure}
    \caption{
	    \label{fig:results-mnist}
	    \textbf{Results on the MNIST dataset.} 
	    In the first column we show the input stroke, where the intensity of the dots goes from black to light grey with increasing time, and the second column is the input image. 
	    The remaining columns show the generated video sequence. 
	    (a) Examples of the same motion stroke applied to four different digits. 
	    The first row is one ground truth example corresponding to the given stroke.  
	    (b) Examples of different motions applied to the same input frame.
	}
    \vspace{-1mm}
\end{figure*}

==> figures/mnist_2.tex <==
\begin{figure*}
	\centering
	\small
	\def\arraystretch{0.1}	
	\newcommand{\height}{6.50cm}
	\newcommand{\vheight}{0.232\height}
	\newcommand{\vsep}{0.05mm}
	% Figure (a)

		\setlength\tabcolsep{1pt}
		\begin{tabular}{lll}
			{\small Stroke} & {\small Image} & \small{Generated frames} \\
			\includegraphics[height=\height]{./images/mnist/a-new/stroke_7.png} &
			\includegraphics[height=\height]{./images/mnist/a-new/input_7.png}&
			\includegraphics[height=\height]{./images/mnist/a-new/frame_7.png} 
		\end{tabular}%
		\setlength\tabcolsep{0.0pt}%
		\begin{tabular}{l}
			{\small Video }
			\vspace{0.5mm} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/b-new/1/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/b-new/3/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/b-new/4/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/a-new/1/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/a-new/2/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/a-new/3/frame}{001}{016} \\
			\animategraphics[height=\vheight,autoplay,loop,poster=last]{5}{./images/mnist/a-new/4/frame}{001}{016} \\
		\end{tabular}

	
    \caption{
	    \label{fig:results-mnist}
	    Results on the MNIST dataset of the same motion stroke applied to different digits and of different motions applied to the same input frame. 
	    The first column shows the input stroke, where the intensity of the dots goes from black to light grey with increasing time, and the second column is the input image. 
	    The remaining columns show the generated video sequence. 
%	    (a) Examples of the same motion stroke applied to four different digits. 
%	    The first row is one ground truth example corresponding to the given stroke.  
%	    (b) Examples of different motions applied to the same input frame.
	}
    \vspace{-1mm}
\end{figure*}
